Equivariant Vector Bundles on Varieties with Codimension-one Orbits

Let $G$ be an algebraic group and let $X$ be a smooth $G$-variety with two orbits: an open orbit and a a closed orbit of codimension $1$. We give an algebraic description of the category of $G$-equivariant vector bundles on $X$ under a mild technical hypothesis. We deduce simpler classifications in the special cases of line bundles and vector bundles which are generically local systems. We apply our results to the study of admissible representations of semisimple Lie groups. Our main result gives a new set of constraints on the associated cycles of unipotent representations.

==> obselete.tex <==
\begin{comment}
	\begin{myproof}{Proof (Lucas)}
		Without loss of generality, we can assume $C$ is the irreducible union of an open $K$-orbit $U$ and a $K$-orbit $Z$ of codimension $1$ in its boundary. Choose an element $e \in Z$, and define the (possibly singular) curve
		%
		$$Y := C \cap S_e$$
		%
		Form the normalization $p: \overline{C}' \to \overline{C}$. Then $\overline{C}'$ decomposes into a single open $K$-orbit $\overline{U}'$ and several closed $K$-orbits $\overline{Z}'_1 \cup ... \cup \overline{Z}'_n$ lying over $\overline{Z}$. Choose any $\overline{Z}'_j$ and an element $\overline{e}_j' \in \overline{Z}_j'$ over $\overline{e}$. By Proposition \ref{prop:fasteningdata}, it suffices to exhibit a fastening datum for $(\overline{U}',\overline{Z}_j')$. 
		
		The one-dimensional torus $\tau(\mathbb{C}^{\times}) \subset K$ acts by scalars on $e$ and therefore fixes its image $\overline{e} \in \overline{C}$. Hence, $\tau$ induces a co-character
		%
		$$\tau: \mathbb{C}^{\times} \hookrightarrow \stab_K(\overline{e})$$
		%
		$\tau(\mathbb{C}^{\times})$ preserves $C$ (by $K$-invariance), $S_e$ (by Proposition \ref{prop:propsofKazhdanaction}(2)), and hence their intersection, $Y$. The $\tau(\mathbb{C}^{\times})$-action on $Y$ descends to a $\tau(\mathbb{C}^{\times})$-action on $\overline{Y}$, which is contracting onto $\overline{e}$ by Proposition \ref{prop:propsofKazhdanaction}(3). In particular, $\tau(\mathbb{C}^{\times})$ acts transitively on the subset $\overline{Y} \setminus \{\overline{e}\}$. 
		
		By functoriality, the $\tau(\mathbb{C}^{\times})$-action on $\overline{Y}$ lifts to a $\tau(\mathbb{C}^{\times})$-action on $p^{-1}(\overline{Y})$, which is transitive on $p^{-1}(\overline{Y} \setminus \overline{e})$ and fixes (pointwise) $p^{-1}(\overline{e})$. Choose any isomorphism $\ell: \BA^1 \cong p^{-1}(\overline{Y} \setminus \overline{e}) \cup \overline{e}_j'$ with $\ell(0) = \overline{e}_j'$. By proposition \ref{prop:propertiesofSlodowy}(1), $\ell$ is transverse to $\overline{Z}_j'$.\todo{This is the sentence that I could not justify without resorting to the above complications. Also, it is not \emph{a priori} clear to me that $p^{-1}(\overline{Y} \setminus \bar{e}) \cup \bar{e}'_j$ is smooth. --James} Hence $(\ell,\tau)$ is a fastening datum for $(\overline{U}',\overline{Z}'_j)$. 
	\end{myproof}
\end{comment}

\begin{comment} 
    \section{Specialization maps} 
	
	Retain the notations and assumptions of Section~\ref{sec:main}. This means that $X = U \cup Z$ is a smooth fastened chain equipped with fastening datum $(\gamma, \ell)$, which determines the group schemes $G^s$ and $\tau_n^*G^s$, the latter being $\gm$-equivariant over $\BA^1$. Theorem~\ref{thm-main} gives us an equivalence between $\QCoh^G_{\tf}(X)$ and a category of filtered co-modules for the filtered Hopf algebra $A = \oh_{G^{s(1)}}$. In this section, we show that some objects in $\QCoh^G_{\tf}(X)$ can be presented more economically, without referring explicitly to $A$. 
	
	\todo{update this} 
	In the first half of this section, we give nicer classifications of line bundles (Proposition~\ref{prop:linebundles}) and sheaves whose restrictions to $U$ are $G$-equivariant local systems (Corollary~\ref{cor-locsys}). These classifications are `nicer' in the sense that the filtered Hopf algebra $A$ does not explicitly appear; instead, in each case $\tilde{G}^s$ acts through a certain quotient $q : \tilde{G}^s \to H$ (see~\ref{s:factor}) for which the specialization to the zero fiber is encoded in a \emph{bona fide} map of algebraic groups $H_0 \to H_1$. In~\ref{sec:univtame} and \ref{s:subcat}, we investigate the largest subcategory which admits such a classification. We show that there is a largest possible quotient of $\tilde{G}^s$ which admits a `specialization map' description (Corollary~\ref{cor-tame-univ}) and we state the corresponding classification of vector bundles in Corollary~\ref{cor-tame-classify}. At the end of the section we compute this largest possible quotient in the case when $\tilde{G}^s$ is a degeneration of $\gm$ to $\BZ/2 \ltimes \ga$. 
	
	For the remainder of this section, we adopt the more concise notation $\tilde{G}^s = \tau_n^*G^s$. Retain the notations $G^{\ell(0)} = \stab_G(\ell(0))$, etc.\ from~\ref{groups}, and recall that $G^{s(0)} \simeq G^s|_0$ and $G^{s(1)} \simeq G^s|_1$, where the fibers are taken with respect to the projection $G^s \to \BA^1$. 
	
	\subsection{Line bundles} \label{s:line}
	
	Let $\Pic^G(X)$ denote the category of $G$-equivariant line bundles on $X$. For any character $\chi : G^{s(1)} \to \gm$, let $\Pic^G_{\chi}(X)$ be the full subcategory consisting of line bundles $\mc{L}$ for which the action $G^{s(1)} \acts \mc{L}|_{s(1)}$ factors through $\chi$. We have a decomposition
	\[
	\Pic^G(X) \simeq \bigsqcup_{\chi} \Pic^G_{\chi}(X).
	\]
	
	\begin{prop}\label{prop:linebundles}
		Fix a character $\chi : G^{s(1)} \to \gm$. 
		\begin{enumerate}[label=(\roman*)]
			\item There exists at most one $\gm$-equivariant map of group schemes $q : \tilde{G}^s \to \gm \times \BA^1$ with the property that $q_1 : G^{s(1)} \to \gm$ equals $\chi$. Such a $q$ exists if and only if $\lim_{t \to 0} \mathrm{Ad}_{\gamma(t^{-1})}^* \chi$ exists as a character on $G^{s(0)}$. 
			\item If $q$ does not exist, then $\Pic^G_{\chi}(X)$ is empty. 
			\item If $q$ exists, then we have a canonical equivalence of groupoids 
			\[
			\Pic^G_{\chi}(X) \simeq (n\BZ + m) \times (\pt / \BC^\times). 
			\]
			The residue class $m \bmod{n}$ is determined by the following property: the restriction of the character 
			\begin{cd}[column sep = 0.8in]
				\gm \ar[r, "\gamma"] & G^{s(0)} \ar[r, "\lim_{t \to 0} \mathrm{Ad}_{\gamma(t^{-1})}^* \chi"] & \gm
			\end{cd}
			to $\mu_n \subset \gm$ is given by $\zeta \mapsto \zeta^m$. 
		\end{enumerate}
	\end{prop}
	\begin{proof}
		Point (i) follows because $\tilde{G}^s$ is flat over $\BA^1$, so a map from $\tilde{G}^s|_{\BA^1 \setminus \{0\}}$ to a separated scheme can admit at most one extension to $\tilde{G}^s$. 
		
		For (ii) and (iii), note that Theorem~\ref{thm-main} implies that an object $\mc{L} \in \Pic^G(X)$ is equivalent to a pair $(\varphi, \mc{L}')$ as follows: 
		\begin{itemize}
			\item $q : \tilde{G}^s \to \gm \times \BA^1$ is a $\gm$-equivariant homomorphism of group schemes over $\BA^1$, where the $\gm$-action on $\gm \times \BA^1$ is via the second factor only. 
			\item $\mc{L}'$ is a $\gm$-equivariant line bundle on $\BA^1$.
			\item We require that the restriction of $\gm \acts \mc{L}'|_{0}$ to $\mu_n$ is given by the group homomorphism $\mu_n \xrightarrow{\gamma} G^s|_{0} \xrightarrow{q_0} \gm$. 
		\end{itemize}
		This is because, for any $\gm$-equivariant line bundle $\mc{L}'$ on $\BA^1$, the group scheme $\curAut_{\BA^1}(\mc{L}')$ is $\gm$-equivariantly isomorphic to $\gm \times \BA^1$, since $\gm$ is abelian. Furthermore, $\mc{L} \in \Pic^G_{\chi}(X)$ if and only if $q_1 = \chi$. 
		
		In case (ii), no such $q$ exists (satisfying $q_1 = \chi$), so $\Pic^G_{\chi}(X)$ is empty. 
		
		In case (iii), there is a unique such $q$, and the remaining datum $\mc{L}'$ amounts to the choice of a one-dimensional vector space (which plays the role of $\mc{L}'|_{1}$) and an integer (which determines the filtration). The third bullet point above says that this integer lies in $n\BZ + m$, because $q_1 = \chi$ implies that $q_0 = \lim_{t \to 0} \mathrm{Ad}_{\gamma(t^{-1})}^* \chi$. 
	\end{proof}
	
	\subsection{Factoring through a quotient of $\tilde{G}^s$} \label{s:factor} 
	
	Let $H$ be another $\gm$-equivariant group scheme over $\BA^1$, and let $q : \tilde{G}^s \to H$ be a map of $\gm$-equivariant group schemes over $\BA^1$. 
	
	\begin{defn}
		Let $\QCoh^{\gm}_{\tf, (n)}(\BA^1 / H)$ be the full subcategory of $\QCoh^{\gm}_{\tf}(\BA^1 / H)$ consisting of sheaves $\mc{F}$ for which the restriction of the action $\gm \ltimes H_0 \acts \mc{F}|_0$ along the group map 
		\[
		q_0 : \gm \ltimes G^{s(0)} \to \gm \ltimes H_0
		\]
		factors through the quotient $\gm \ltimes G^{s(0)} \to G^{\ell(0)}$. 
	\end{defn}
	
	\begin{prop}\label{flat-tame-prop}
		We have the following: 
		\begin{enumerate}[label=(\roman*)]
			\item If $q_1 : G^{s(1)} \to H_1$ is surjective and $H$ is flat (i.e.\ torsion-free) over $\BA^1$, then the pullback functor 
			\[
			\QCoh^{\gm}_{\tf, (n)}(\BA^1 / H) \xrightarrow{q^*}  \QCoh^{\gm}_{\tf, (n)}(\BA^1 / \tilde{G}^s)
			\]
			is fully faithful. 
			\item If furthermore $q_0 : G^{s(0)} \to H_0$ is surjective, then the image of this functor is the subcategory of sheaves $\mc{F}$ for which the action $G^{s(1)} \acts \mc{F}|_1$ factors through $q_1$. 
		\end{enumerate}
	\end{prop}
	\begin{proof}
		(i). Since $H$ is flat, an object in the left hand side is given by $(V, F, \beta)$ where $(V, F)$ is a filtered vector space and $\beta : V \to V \otimes \oh_{H_1}$ is a filtered coaction. Since $q_1$ is surjective, $\oh_{H_1} \to \oh_{G^{s(1)}}$ is injective, so whether or not a filtered coaction $V \to V \otimes \oh_{G^{s(1)}}$ factors through a coaction $V \to V \otimes \oh_{H_1}$ is a property, not additional structure. 
		
		(ii). The crux of the proof is the following lemma, which the second author learned from Dori Bejleri: 
		\begin{lem*}
			Let $f : X \to Y$ be a map of schemes over a base $S$. Let $x \in X$ be a point, and let $y \in Y$ and $s \in S$ be its images. Then the following two statements are equivalent: 
			\begin{enumerate}[label=(\roman*)]
				\item $X\to S$ is flat at $x$, and $f|_s : X|_s \to Y|_s$ is flat at $x$. 
				\item $Y \to S$ is flat at $y$, and $f$ is flat at $x$. 
			\end{enumerate}
		\end{lem*} 
		Since $q_0$ is a surjective map of algebraic groups, it is flat. Since $\tilde{G}^s$ is flat over $\BA^1$, we may apply the lemma and conclude that $q$ is flat. Since flat maps are preserved by base change, we conclude that the scheme $\ker(q)$ is flat over $\BA^1$. 
		
		The image of the functor is obviously contained in the indicated subcategory. For the reverse containment, suppose that the sheaf $\mc{F} \in \QCoh^{\gm}_{\tf, (n)}(\BA^1 / \tilde{G}^s)$ lies in the indicated subcategory. The action of $\tilde{G}^s$ corresponds to a map $\tilde{G}^s \xrightarrow{\varphi} \curEnd_{\BA^1}(\mc{F})$. The closed subscheme $\ker(\varphi)|_{\BA^1 \setminus \{0\}}$ contains $\ker(q)|_{\BA^1 \setminus \{0\}}$ by the hypothesis on $\mc{F}$. The flatness proved in the previous paragraph implies that $\ker(\varphi)$ contains $\ker(q)$. Therefore the action of $\tilde{G}^s$ factors through $q$, as desired. 
	\end{proof}
	
	\begin{defn}\label{def-q-cat} 
		As a notational convenience, when the hypotheses of Proposition~\ref{flat-tame-prop}(i) are satisfied, we define $\QCoh^{G}_{\tf, q}(X)$ via the following Cartesian diagram: 
		\begin{cd}
			\QCoh^{G}_{\tf, q}(X) \ar[r, hookrightarrow] \ar{d}[rotate=90, anchor=south, swap]{\sim} & \QCoh^{G}_{\tf}(X) \ar{d}[rotate=90, anchor=south, swap]{\sim}{\text{Thm.~\ref{thm-main}}} \\
			\QCoh^{\gm}_{\tf, (n)}(\BA^1 / H) \ar[r, hookrightarrow, "q^*"] & \QCoh^{\gm}_{\tf, (n)}(\BA^1 / \tilde{G}^s)
		\end{cd}
		Note that this subcategory of $\QCoh^{G}_{\tf, (n)}(X)$ \emph{a priori} depends on the choice of fastening $(\gamma, \ell)$ as well as the map $q$. But when Proposition~\ref{flat-tame-prop}(ii) applies, it tells us that this subcategory consists exactly of those sheaves $\mc{F} \in \QCoh^G_{\tf}(X)$ for which the action $G^{s(1)} \acts \mc{F}$ factors through $q_1$. 
		
		This definition will appear only in Corollary~\ref{cor-tame-classify}. 
	\end{defn}
	
	\subsection{Local systems} \label{s:locsys}
	
	We apply~\ref{s:factor} to the problem of describing the subcategory 
	\[
	\QCoh_{\tf, \locsys}^G(X) \hra \QCoh_{\tf}^G(X) 
	\]
	consisting of sheaves $\mc{F}$ for which the restriction $\mc{F}_U$ is a $G$-equivariant local system. 
	
	We construct a quotient map $q : \tilde{G}^s \to H_{\locsys}$ of group schemes over $\BA^1 / \gm$ as follows. For each connected (equivalently, irreducible) component $C \subset \tilde{G}^s$, let $H_C \to \BA^1$ be the image of the projection map $C \to \BA^1$. Since $\tilde{G}^s$ is flat over $\BA^1$, each $H_C$ is either $\BA^1$ or $\BA^1 \setminus \{0\}$. We define 
	\[
	H_{\locsys} := \bigsqcup_{\substack{C \subset \tilde{G}^s \\ \text{components}}} H_C. 
	\]
	Then $H_{\locsys}$ is obviously a group scheme over $\BA^1 / \gm$, and the desired map $q$ is defined on components by the tautological map $C \to H_C$. Note that $H_1 \simeq \on{Com}(G^{s(1)})$ where $\on{Com}(-)$ means the group of components. 
	
	Since each component of $G^{s(0)}$ lies in a unique component of $\tilde{G}^s$, and the latter components are in bijection with those of $G^{s(1)}$, we obtain a canonical map of groups 
	\[
	\sigma : \on{Com}(G^{s(0)}) \to \on{Com}(G^{s(1)}). 
	\]	
	
	\begin{cor}\label{cor-locsys}
		Let $\mc{C}_{\locsys, (n)}(X)$ be the category whose objects are triples $(V, F, \rho)$ as follows: 
		\begin{itemize}
			\item $V$ is a vector space, $\rho : \on{Com}(G^{s(1)}) \acts V$ is a representation, and $F$ is an exhausting filtration on $V$ which is invariant under $\rho$. 
			\item We furthermore require that the restriction of the associated graded action 
			\[
			\gm \ltimes G^{s(0)} \to \gm \times \on{Com}(G^{s(0)}) \xrightarrow{\sigma} \gm \times \on{Com}(G^{s(1)}) \acts \gr^F V
			\]
			factors through the quotient $\gm \ltimes G^{s(0)} \sra G^{\ell(0)}$. 
		\end{itemize}
		The morphisms in this category are maps of filtered representations. Then there is an equivalence of categories
		\[
		\QCoh^G_{\tf, \locsys}(X) \simeq \mc{C}_{\locsys, (n)}(X). 
		\]		
	\end{cor}
	\begin{proof}
		Since Proposition~\ref{flat-tame-prop}(ii) applies to $q : \tilde{G}^s \to H_{\locsys}$, we conclude that the category $\QCoh^{\gm}_{\tf, (n)}(\BA^1 / H_{\locsys})$ is equivalent to the subcategory of $\QCoh^{\gm}_{\tf, (n)}(\BA^1 / \tilde{G}^s)$ consisting of sheaves $\mc{F}$ for which the action $G^{s(1)} \acts \mc{F}|_1$ factors through $G^{s(1)} \sra \on{Com}(G^{s(1)})$. But this subcategory is also equivalent to $\QCoh^G_{\tf, \locsys}(X)$ by Theorem~\ref{thm-main}. Thus, to finish the proof, it suffices to show that 
		\[
		\mc{C}_{\locsys, (n)}(X) \simeq \QCoh^{\gm}_{\tf, (n)}(\BA^1 / H_{\locsys}).
		\]
		
		The right hand side consists of triples $(V, F, \beta)$ where $(V, F)$ is as before, and $\beta : V \to V \otimes \oh_{H_{\locsys}|_1}$ is a filtered coaction. We observed above that $H_{\locsys}|_1 \simeq \on{Com}(G^{s(1)})$. If $I \subset \oh_{\on{Com}(G^{s(1)})}$ is the ideal of the subscheme $\Im(\sigma)$, then the filtration on this Hopf algebra is given by
		\begin{equation} \label{filt}
		F^{\ge m} \oh_{\on{Com}(G^{s(1)})} = \begin{cases}
		\oh_{\on{Com}(G^{s(1)})} & \text{ if } m \le 0 \\
		I & \text{ if } m > 0. 
		\end{cases}
		\end{equation}
		It is immediate to check using the definition of $H_{\locsys}$ that it corresponds to $(\oh_{\on{Com}(G^{s(1)})}, F)$ under the Artin--Rees construction. This explicit description of the filtration on $\oh_{\on{Com}(G^{s(1)})}$ implies that the filtered coaction $\beta$ is equivalent to the data in the first bullet point in the definition of $\mc{C}_{\locsys, (n)}(X)$. It is easy to check that the second bullet point corresponds to the $(-)_{(n)}$ condition on the right hand side. 
	\end{proof}
	
	
	\subsection{The universal tame quotient}\label{sec:univtame}
	
	The analysis in~\ref{s:line} and \ref{s:locsys} is especially nice because in both cases we considered a quotient $q : \tilde{G}^s \to H$ (in the framework of~\ref{s:factor}) with the property that $H \to \BA^1$ is `almost' a constant group scheme. Indeed, in~\ref{s:line}, $H$ was the constant group scheme $H \simeq \gm \times \BA^1$. And in~\ref{s:locsys}, $H_{\locsys}$ is obtained from the constant group scheme $\on{Com}(G^{s(1)}) \times \BA^1$ by replacing the zero fiber by its closed subscheme $\Im(\sigma)$. In the proof of Corollary~\ref{cor-locsys}, we saw that this `almost constant' behavior over $\BA^1 / \gm$ is encoded by the filtration~\ref{filt}. 
	
	In the remainder of this section, we pursue this idea in greater generality. 
	
	\begin{defn}
		A filtered vector space $(V, F)$ is \emph{tamely filtered} if $F^{\ge 0} V= V$ and $F^{\ge 1} V = F^{\infty}V$.\footnote{By definition, $F^\infty V = \bigcap_{m \in \BZ} F^{\ge m} V$ and $F^{-\infty} V = \bigcup_{m \in \BZ} F^{\ge m} V$. The filtration $F$ is exhausting if and only if $F^{-\infty} V = V$.} Let $\QCoh_{\tf, \tame}^{\gm}(\BA^1)$ be the full subcategory of $\QCoh_{\tf}^{\gm}(\BA^1)$ corresponding under the Artin-Rees construction to tamely filtered vector spaces.\footnote{Note that $\QCoh_{\tf, \tame}^{\gm}(\BA^1)$ is equivalent to the category of pairs $(V, V')$ where $V$ is a vector space and $V' \subset V$ is a subspace.} 
	\end{defn}
	
	Since this is a monoidal subcategory, we obtain an analogous notion of tame affine schemes over $\BA^1 / \gm$ as in the remark after Proposition~\ref{ar}. (Note that a tame affine scheme is by definition flat over $\BA^1$.) Let us describe this notion in more detail. Any (flat) affine scheme over $\BA^1 / \gm$ is given by 
	\[
	\ul{\Spec} (R, F) := \Spec \oplus_m F^{\ge m} R \xrightarrow{\pi} \Spec k[h] = \BA^1
	\]
	for some filtered ring $(R, F)$. Here $\oplus_m F^{\ge m} R$ and $k[h]$ are graded rings with $\oplus_m F^{\ge m} R$ in degree $m$ and $h$ in degree $-1$. (This convention ensures that the action $\gm \acts \BA^1_h$ is standard.) Then $\pi$ is defined by $h \mapsto 1_R \in F^{\ge -1} R$. 
	
	We call this affine scheme \emph{tame} if $(R, F)$ is tamely filtered. In particular, any tame affine scheme is by definition torsion-free (equivalently flat) over $\BA^1$. 
	
	Next, we observe that tame affine schemes are `almost constant' as described in the first paragraph of this subsection. For a vector space $V$, let $F_0$ be the filtration for which $F_0^{\ge 0} = V$ and $F_0^{\ge 1}V = 0$. 
	
	\begin{lem}	\label{tame-describe} 
		We have the following. 
		\begin{enumerate}[label=(\roman*)]
			\item The map of filtered rings $(F^{\ge 0} R, F_0) \to (R, F)$ yields a map 
			\[
			\ul{\Spec} (R, F) \xrightarrow{p} (\Spec R) \times \BA^1. 
			\]
			of schemes over $\BA^1 / \gm$, where the $\gm$-action on the target is via the second factor only, with the standard action. 
			\item If $(R, F)$ is tamely filtered, then the base change of $p$ along $\BA^1 \setminus \{0\} \hra \BA^1$ is an isomorphism and the base change along $\{0\} \hra \BA^1$ is the closed embedding $\Spec R/F^{\ge 1} R \hra \Spec R$. In particular, there is a canonical map from the zero fiber of $\Spec (R, F)$ to the general fiber. 
		\end{enumerate}
	\end{lem}
	\begin{proof}
		Point (i) is a tautology. For point (ii), if $(R, F)$ is tamely filtered, then $R = F^{\ge 0} R$, from which it follows that $p$ is an isomorphism over $\BA^1 \setminus \{0\}$. The base change of $p$ along $\{0\} \hra \BA^1$ is the induced map on associated graded rings, which is $R \sra R / F^{\ge 1} R$ if $(R, F)$ is tamely filtered. 
	\end{proof}
	
	Tame affine schemes over $\BA^1$ are usually not finite type. For example, let $R = k[x]$ and $F^{\ge 1}R = \la x \ra$. Then $\oplus_m F^{\ge m} R \simeq k[h, h^{-1}x, h^{-2}x, \cdots]$ which is not finitely generated. (Geometrically, this ring can be constructed from the plane $\Spec k[h, x]$ by taking an infinite sequence of affine charts of blow-ups at the origin, the first of which is $k[h, x] \to k[h, h^{-1}x]$.) The following lemma tells us what finite type tame affine schemes look like: 
	
	\begin{lem} \label{tame-describe-2} 
		Let $(R, F)$ be a tamely filtered $k$-algebra. 
		\begin{enumerate}[label=(\roman*)]
			\item $\oplus_m F^{\ge m} R$ is finitely generated (as a $k$-algebra) if and only if $R$ is finitely generated and the ideal $F^{\ge 1} R$ is idempotent. 
			\item If the situation of (i) obtains, then the map $p$ from Lemma~\ref{tame-describe} looks as follows. Over each connected component $C \subset \Spec R$, the map $p$ is either the identity map of $C \times \BA^1$ or the open embedding $C \times (\BA^1 \setminus \{0\}) \hra C \times \BA^1$. The former occurs if and only if $F^{\ge 1}R$ vanishes on $C$. 
		\end{enumerate}
	\end{lem}
	\begin{proof}
		(i). If $\oplus_m F^{\ge m} R$ is finitely generated, choose a finite set of homogeneous generators, and partition them into two groups $\{r_i\} \cup \{s_j\}$ where the $r_i$ live in nonpositive degrees and the $s_j$ live in positive degrees. Let $n$ be the largest degree which occurs among the generators. For degree reasons, every polynomial in the generators which lies in the summand $F^{\ge n+1} R$ must be a sum of monomials each of which contains at least two $s_j$'s. The $s_j$'s lie in $F^{\ge 1}R$ when viewed as elements of $R$ (i.e.\ forgetting the grading). Therefore 
		\[
		F^{\ge 1} R = F^{\ge n+1} R \subset (F^{\ge 1} R)^2
		\]
		as ideals of $R$. (The equality uses the tamely filtered hypothesis.) Hence $F^{\ge 1} R$ is idempotent. Also, the fiber of $\Spec \oplus_m F^{\ge m} R \xrightarrow{\pi} \Spec k[h]$ at $h=1$ is $\Spec R$, so $R$ is also finitely generated. 
		
		Conversely, assume that $F^{\ge 1} R$ is idempotent and $R$ is finitely generated. Since $R$ is Noetherian, $F^{\ge 1} R$ is a finitely generated ideal. A set of generators for $\oplus_m F^{\ge m} R$ is given by taking a set of generators for $R$ placed in degree 0, a set of ideal generators for $F^{\ge 1} R$ placed in degree $1$, and the element $1_R$ placed in degree $-1$. 
		
		Point (ii) is deduced from Lemma~\ref{tame-describe} and the fact that an idempotent ideal of a Noetherian ring vanishes on a union of connected components. 
	\end{proof}
	
	Next, we observe that every filtered ring has a universal tame quotient. 
	
	\begin{lem} \label{lem-tame-cat} 
		The subcategory $\QCoh^{\gm}_{\tf, \tame}(\BA^1)$ is colocalizing, i.e.\ there are adjoint functors
		\[
		\iota : \QCoh^{\gm}_{\tf, \tame}(\BA^1) \rightleftarrows \QCoh^{\gm}_{\tf}(\BA^1) : \tau_{\tame}
		\]
		where $\iota$ is the inclusion and $\tau_{\tame}$ sends $(V, F)$ to $(F^{\ge 0} V, F_1)$ where $F_1$ is the tame filtration defined by $F_1^{\ge m}  = F^{\infty} V$ for all $m > 0$. Both of these functors are monoidal. 
	\end{lem}
	\begin{proof}
		Omitted. 
	\end{proof}
	
	\begin{cor}\label{cor-tame} %\todo{James: again, do you want these schemes to be torsion-free over A1?}
		The subcategory $\Sch_{\BA^1 / \gm}^{\on{aff}, \tame} \subset \Sch^{\on{aff}}_{\BA^1 / \gm}$ of tame affine schemes is localizing, i.e.\ there are adjoint functors 
		\[
		\tau^{\tame} : \Sch_{\BA^1 / \gm}^{\on{aff}} \rightleftarrows \Sch_{\BA^1 / \gm}^{\on{aff}, \tame} : \iota
		\]
		where $\iota$ is the inclusion. The functor $\tau^{\tame}$ preserves the class of affine schemes whose every connected component is integral and finite type. 
	\end{cor}
	\begin{proof}
		The last sentence is not obvious. It suffices to show that, if $\oplus_m F^{\ge m} R$ is finitely generated and integral, then the following statements hold: 
		\begin{enumerate}[label=(\roman*)]
			\item The subring $F^{\ge 0} R$ is finitely generated. 
			\item The ideal $F^{\infty} R$ is either $\la 0 \ra$ or $F^{\ge 0} R$.\footnote{In the latter case, $F$ must be the trivial filtration satisfying $F^{\ge m} R = R$ for all $m$.} 
		\end{enumerate}
		This is because of Lemma~\ref{tame-describe-2}(i) and the fact that we can consider each connected component separately. 
		
		Let $s_i$ for $i = 1, \ldots, r$ be a finite set of homogeneous generators for the graded ring $\oplus_m F^{\ge m} R$. Then we have 
		\[
		F^{\ge m} R = \underset{\substack{e_1, \ldots, e_r \ge 0\\ \Sigma_i\, e_i \deg(s_i) = m}}{\on{span}}  \left(\underset{i=1}{\overset{r}{\Pi}} s_i^{e_i} \right)
		\]
		where the notation means span over $k$. In particular, the monomials of degree zero are in bijection with the kernel of the map of monoids $\BN^{\oplus r} \xrightarrow{\on{deg}} \BZ$ which sends $(e_1, \ldots, e_r) \mapsto \sum_{i} e_i \deg(s_i)$. A basic lemma (often used in toric geometry) says that any submonoid of $\BZ^{\oplus r}$ which is cut out by linear inequalities with \emph{rational} coefficients is finitely generated \todo{James: can you find a reference for this?}. This implies (i). 
		
		Similarly, applying the lemma to the submonoid of $\BN^{\oplus r}$ cut out by the inequality $\deg \ge 0$ yields a finite set of generators of $\oplus_{m \ge 0} F^{\ge m} R$, which we may denote $t_1, \ldots, t_{\ell}$, with $\on{deg}(t_i) \ge 0$. If all these degrees are zero, then $F^{\ge m} R = \la 0 \ra$ for $m > 0$, which proves (ii). Therefore, we may assume that not all degrees are zero. Let $\ell_0$ be a cutoff such that $\deg(t_i) > 0$ if and only if $i \le \ell_0$. Then 
		\[
		F^{\ge m} R = \sum_{\substack{e_1, \ldots, e_{\ell_0} \ge 0\\ \Sigma_i\, e_i \deg(t_i) = m}} \left \langle \underset{i=1}{\overset{\ell_0}{\Pi}} t_i^{e_i} \right \rangle
		\]
		where $\langle-\rangle$ denotes an ideal in $F^{\ge 0} R$. On the other hand, define 
		$
		I = \langle t_1, \ldots, t_{\ell_0} \rangle, 
		$
		so that 
		\[
		I^m = \sum_{\substack{e_1, \ldots, e_{\ell_0} \ge 0\\ \Sigma_i\, e_i = m}} \left \langle \underset{i=1}{\overset{\ell_0}{\Pi}} t_i^{e_i} \right \rangle
		\]
		Let $d := \max_i \deg(t_i) > 0$. Then we have 
		\[
		I^m \subset F^{\ge m} R \subset I^{\lfloor \frac{m}{d} \rfloor}, 
		\]
		because we have the implications 
		\[
		\Sigma_i\, e_i \ge m \quad \Longrightarrow \quad \Sigma_i\,  e_i \deg(t_i)\ge m \quad \Longrightarrow \quad \Sigma_i\, e_i d \ge m. 
		\]
		Taking intersections over all $m$ implies that $F^{\infty} R = \cap_m I^m$. Since $R$ is integral by hypothesis, the Krull Intersection Theorem implies that $F^\infty R$ is either $\la 0 \ra$ or $F^{\ge 0}R$, as desired. 
	\end{proof}
	
	We shall omit instances of $\iota$ in the subsequent notation. 
	
	\begin{cor} \label{cor-tame-univ}
		There is a finite type flat affine group scheme $\tau^{\tame}(\tilde{G}^s)$ over $\BA^1 / \gm$ and a map $q : \tilde{G}^s \to \tau^{\tame}(\tilde{G}^s)$ of group schemes over $\BA^1/\gm$ which is initial for all such maps from $\tilde{G}^s$ to a \underline{tame} affine group scheme over $\BA^1 / \gm$. The map $q$ is dominant because $q_1$ is surjective. 
	\end{cor}
	\begin{proof}
		This follows from Corollary~\ref{cor-tame} and the monoidality noted in Lemma~\ref{lem-tame-cat}. For the last sentence, note that $q_1$ is dominant because $F^{\ge 0} R \to R$ is an injection for any filtered ring $(R, F)$, and this implies that $q_1$ is surjective because it is a map of group schemes. 
	\end{proof}
	
	In view of Lemma~\ref{tame-describe-2}(ii), $\tau^{\tame}(\tilde{G}^s)$ can be described very concretely: it consists of a group $G^{\tame}_1$ and a subgroup $G^{\tame}_0$ corresponding to a subset of the connected components. The former is the general fiber and the latter is the special fiber of $\tau^{\tame}(\tilde{G}^s)$. There is a canonical surjective\footnote{The universal property of $\tau^{\tame}(-)$ implies that this map is dominant as a map of varieties. Since it is a homomorphism of algebraic groups, it must therefore be surjective.} map $G^{s(1)} \sra G^{\tame}_1$ and a canonical $\gm$-equivariant map $G^{s(0)} \to G^{\tame}_0$, where the $\gm$-action on the target is trivial.
	
	By construction, $\tau^{\tame}(\tilde{G}^s)$ is the `universal' example of a family of quotients of the fibers of $\tilde{G}^s$, for which the geometric relationship of specialization to the zero fiber is encoded by an actual map of groups: 
	\begin{cd}[column sep = 1.3in] 
		G^{s(1)} \ar[d, twoheadrightarrow, "{\mathrm{surjective}}"] & G^{s(0)} \ar[d, "\gm\text{-equivariant}"] \\
		G^{\tame}_1 \ar[hookleftarrow]{r}{\text{incl.\ of components}}[swap]{\text{Lemma~\ref{tame-describe}(ii)}} & G^{\tame}_0
	\end{cd}
	
	\begin{rmk}
		Using the proof of Proposition~\ref{prop:linebundles} and the universal property of $\tau^{\tame}(\tilde{G}^s)$, we conclude that a character $\chi : G^{s(1)} \to \gm$ is good in the sense of Proposition~\ref{prop:linebundles}(i) if and only if it factors through $G^{s(1)} \sra G_1^{\on{tame}}$. In this case, the character $\lim \chi$ of $G^{s(0)}$ can be computed as the composition 
		\[
		G^{s(0)} \to G_0^{\on{tame}} \hra G_1^{\on{tame}} \xrightarrow{\chi} \gm. 
		\]
		In effect, the computation of the limit character in Proposition~\ref{prop:linebundles} is encapsulated in the construction of the tame quotient, which contains information about the limits of all functions on $G^{s(1)}$ under specialization toward the zero fiber. 
	\end{rmk}
	
	
	\subsection{The subcategory associated to a tame quotient} \label{s:subcat}
	
	Let us apply~\ref{s:factor} to a map $q : \tilde{G}^s \to H$ where $H$ is tame. For example one could take $q$ to be the universal map produced by Corollary~\ref{cor-tame-univ}. We deduce the following generalization of Corollary~\ref{cor-locsys}: 
	\begin{cor}\label{cor-tame-classify}
		Let $\mc{C}_{q, (n)}(X)$ be the category whose objects are triples $(V, F, \rho)$ as follows: 
		\begin{itemize}
			\item $V$ is a vector space, $\rho : H_1 \acts V$ is a representation, and $F$ is an exhausting filtration on $V$ which is invariant under $\rho$. 
			\item We furthermore require that the restriction of the associated graded action 
			\[
			\gm \ltimes G^{s(0)} \to \gm \times H_0 \xrightarrow{\sigma} \gm \times H_1 \acts \gr^F V
			\]
			factors through the quotient $\gm \ltimes G^{s(0)} \sra G^{\ell(0)}$. Here the map $\sigma$ arises from Lemma~\ref{tame-describe}(ii). 
		\end{itemize}
		The morphisms in this category are maps of filtered representations. Then there is an equivalence of categories
		\[
		\QCoh^G_{\tf, q}(X) \simeq \mc{C}_{q, (n)}(X)
		\]	
		where the left hand side is as in Definition~\ref{def-q-cat}. 
	\end{cor}
	\begin{proof}
		The proof is identical to that of Corollary~\ref{cor-locsys}. 
	\end{proof}
	
	Recall that Proposition~\ref{flat-tame-prop}(ii) gives a criterion under which the subcategory $\QCoh^G_{\tf, q}(X) \subset \QCoh^G_{\tf}(X)$ can be characterized in terms of the behavior of a sheaf $\mc{F} \in \QCoh^G_{\tf}(X)$ on $U$. Thus, when this criterion is satisfied, we have a subcategory for which it is easy to detect membership and to classify objects. Unfortunately, the closer $q$ is to being `universal,' the less likely it is to satisfy this criterion. 
	
	\begin{ex}
		In closing, we illustrate the preceding notions by constructing an example of a family of groups over $\BA^1$ which plays the role of $\tilde{G}^s$ and a tame quotient of this family which fails the criterion of Proposition~\ref{flat-tame-prop}(ii). Let $G = \GL_2$ and define the $\gm$-action on $G \times \BA^1$ via conjugation by the subgroup $\gamma : \gm \hra G$ defined by $\gamma(t) = \begin{pmatrix} 1 & 0 \\ 0 & t \end{pmatrix}$. Define the closed subscheme $\tilde{G}^s \subset G \times \BA^1$ by requiring that 
		\[
		\tilde{G}^s|_1 = \left\{ \left. \begin{pmatrix}
		a & b \\ b & a 
		\end{pmatrix}\ \right|\ a^2 - b^2 = 1 \right\}, 
		\]
		that $\tilde{G}^s$ is invariant under the $\gm$-action, and that it is flat over $\BA^1$. This implies that  
		\[
		\tilde{G}^s|_t = \left\{ \left. \begin{pmatrix}
		a & bt^{-1} \\ bt & a 
		\end{pmatrix}\ \right|\ a^2 - b^2 = 1 \right\} 
		\]
		for all $t\neq 0$, and 
		\[
		\tilde{G}^s|_0 = \left\{ \left. \begin{pmatrix}
		a & c \\ 0 & a 
		\end{pmatrix}\ \right|\ a^2 = 1 \right\}. 
		\]
		Thus, $\tilde{G}^s$ is a degeneration from the group $\gm$ to the group $\BZ / 2 \ltimes \ga$. 
		
		Next, we find the universal tame quotient $\tilde{G}^s \to \tau^{\tame}(\tilde{G}^s)$. We have $A \simeq \oh_{\tilde{G}^s|_1} \simeq k[a, b] / \la a^2 - b^2 - 1\ra$, and the filtration on $A$ is the $\la b \ra$-adic filtration, meaning that 
		\[
		F^{\ge m} A = \begin{cases}
		A & \text{ if } m \le 0 \\
		\la b \ra^m & \text{ if } m > 0. 
		\end{cases}
		\]
		Since $\cap_m \la b \ra^m = \la 0 \ra$, we have 
		\[
		F^{\ge m} \tau^{\tame} A = \begin{cases}
		A & \text{ if } m \le 0 \\
		\la 0 \ra & \text{ if } m > 0. 
		\end{cases}
		\]
		Thus $\tau^{\tame}(\wt{G}^s) \simeq \gm \times \BA^1$. The map $G^s|_1 \sra G_1^{\tame}$ is an isomorphism, while the map $G^s|_0 \to G_0^{\tame}$ is the composition
		\[
		\BZ/2 \ltimes \ga \sra \BZ / 2 \hra \gm. 
		\]
		Thus the universal tame quotient is \emph{not} flat in the sense of Proposition~\ref{flat-tame-prop}. In fact, the only flat tame quotient of $\tilde{G}^s$ is the trivial one. 		
		
		The characterization of the filtration on $A$ as the $\la b \ra$-adic filtration allows one to say a bit more. The group scheme $\wt{G}^s$ is obtained from the constant family $\gm \times \BA^1$ via deformation to the normal cone applied to the subgroup 
		\[
		\{\pm 1\} = V(b) \hra \Spec A \simeq \gm. 
		\]
		In general, given a group $G$ and a subgroup $H$, the deformation to the normal cone of $H$ in $G$ yields a $\gm$-equivariant degeneration from $G$ to the normal bundle $\mc{N}_{H/G}$. (The group structure of the normal bundle is given by its realization as $\mc{N}_{H/G}|_1 \rtimes H$.) The degeneration from the Poincar\'e group to the Galilean group is realized in this way. 
	\end{ex}
\end{comment} 




\begin{comment}
	\subsubsection{The graph of a chain} 
	\todo{James: if I'm understanding correctly, Uj always refers to a G-orbit on the normalization? If so, would it make sense to put tildes over the Ujs for consistency?}
	Preserve the notation of~\ref{weak}, so $G \acts X$ is a chain. We introduce some notation to keep track of the adjacency relations between open and closed $G$-orbits. Define a bipartite directed graph $\Gamma$ as follows: 
	\begin{itemize}
		\item The vertex set is the set of $G$-orbits on $X$. 
		\item For each pair $(U_j, \wt{Z}_i)$ where $U_j$ is a $G$-orbit on $\wt{X}$ and $\wt{Z}_i$ is a $G$-orbit in the boundary of $U_j$, we have one edge from $U_j$ to $Z_i$, where $Z_i$ is the image of $\wt{Z}_i$ under the map $\wt{Z} \to Z$. 
	\end{itemize}
	Define another bipartite directed graph $\Gamma'$ as follows: 
	\begin{itemize}
		\item The vertex set is $S_U \sqcup S_Z \sqcup S_{\wt{Z}} \sqcup \on{Edges}(\Gamma)$ where the first three terms refer to the set of $G$-orbits in $U, Z, \wt{Z}$, and the last term is the set of edges of $\Gamma$. 
		\item For every $e = (U_j, \wt{Z}_i) \in \on{Edges}(\Gamma)$, there are edges $U_j \to e$ and $\wt{Z}_i \to e$. 
		\item For each $\wt{Z}_i \in S_{\wt{Z}}$, there is an edge $\wt{Z}_i \to Z_k$ where $Z_k$ is the image of $\wt{Z}_i$ under $\nu$. 
	\end{itemize}
	There is a functor $F : (\Gamma')^{\op} \to \on{Chains}_G$ defined as follows: 
	\begin{itemize}
		\item A vertex of $\Gamma'$ which corresponds to an edge $e = (U_j, \wt{Z}_i)$ of $\Gamma$ goes to the $G$-chain given by $U_j \cup \wt{Z}_i$ as a locally closed subvariety of $\wt{X}$. 
		\item Every other vertex of $\Gamma'$ goes to the corresponding $G$-orbit. 
	\end{itemize}
	The behavior of $F$ on morphisms is clear. 
	
	\begin{prop}\label{weak-prop-2} 
		If $X$ is weakly normal, then the limit of the diagram of categories given by $\Vect^G(-) \circ F^{\op} : (\Gamma')^{\op} \to \on{Cat}$ is equivalent to $\Vect^G(X)$. 
	\end{prop}
	\begin{proof}
		Fix $U_j \in S_U$, and let $\wt{Z}_i$ range over all orbits in the boundary of $U_j$. The induced subgraph of $\Gamma'$ given by the vertices $U_j$ and $(U_j, \wt{Z}_i)$ is connected to the rest of $\Gamma'$ only via the edges $(U_j, \wt{Z}_i) \to \wt{Z}_i$ for each $i$. The limit of categories associated to this induced subgraph is $\Vect^G(\ol{U}_j)$ because the $U_j \cup \wt{Z}_i$ constitute an open cover of $\ol{U}_j$. Thus, we may contract this subgraph to a single vertex $v_{U_j}$ which is associated to the category $\Vect^G(\ol{U}_j)$ without changing the desired limit of categories. (Each edge $v_{U_j} \to \wt{Z}_i$ corresponding to the edge $(U_j, \wt{Z}_i)$ is associated to the functor $\Vect^G(\ol{U}_j) \to \Vect^G(\wt{Z}_j)$ given by restriction.) 
		
		The product of the categories associated to the $v_{U_j}$ (for all $U_j \in S_U$) is equivalent to $\Vect^G(\wt{X})$. The product of the categories associated to the vertices $\wt{Z}_i$ is equivalent to $\Vect^G(\wt{Z})$. And the product of the categories associated to the vertices $Z_i \in S_Z$ is equivalent to $\Vect^G(Z)$. Now it is easy to see (using the connectivity pattern of the graph obtained from $\Gamma'$ via the previous paragraph) that the desired limit of categories coincides with that of Proposition~\ref{weak-prop}(iii), as desired. 
	\end{proof}
	
	\begin{rmk}
		Concretely, this means that a $G$-equivariant vector bundle on $X$ is equivalent to the following data: 
		\begin{itemize}
			\item We choose $V_k \in \Vect^G(Z_k)$ for each $Z_k \in S_Z$. 
			\item We choose $W_j \in \Vect^G(U_j)$ for each $U_j \in S_U$. 
			\item For each $(U_j, \wt{Z}_i)$ where $\wt{Z}_i$ is in the boundary of $U_j$ in $\wt{X}$, we choose an object $E \in \Vect^G(U_j \cup \wt{Z}_i)$ along with isomorphisms between its restriction to $U_j$ and $W_j$, and between its restriction to $\wt{Z}_i$ and the pullback of $V_k$ to $\wt{Z}_i$ (where $k$ is such that $\wt{Z}_i$ maps to $Z_k$). 
		\end{itemize}
		Since there are no two-dimensional cells in $\Gamma'$, cocycle conditions do not appear in the above list. This is a convenient consequence of the `codimension zero or one' requirement in the definition of a chain. 
		
		Of course, if we choose basepoints $z_i \in Z_i$ and $u_j \in U_j$, then we have equivalences $\Vect^G(Z_i) \simeq \on{Rep}(\stab_G(z_i))$ and $\Vect^G(U_j) \simeq \on{Rep}(\stab_G(u_j))$. Theorem~\ref{thm-main} describes the category $\Vect^G(U_j \cup \wt{Z}_i)$. 
	\end{rmk}
	
	\begin{cor}
	    If $X$ is weakly normal and $\Gamma'$ is contractible,\footnote{This means that the topological space associated to $\Gamma'$ is contractible, i.e.\ the directed graph $\Gamma'$ does not contain a `zig-zag cycle.'} then the assertion of Proposition~\ref{weak-prop-2} also holds at the level of isomorphism classes. 
	\end{cor} 
	
	\begin{rmk}
    	If $\Gamma'$ is contractible, then $\Gamma$ is contractible, but the converse is not true. 
	\end{rmk}
	
\section{Line Bundles: Revisited}\label{sec:linebundles}

Let $X = U_1 \cup ... \cup U_m \cup Z_1 \cup ... Z_n$ be a weakly normal, fastened $G$-chain. Write
%
$$\tilde{X} = \tilde{U}_1 \cup ... \cup \tilde{U}_m \cup \bigcup_{k_1 =1}^{p_1} \tilde{Z}_1^{k_1} \cup ... \cup \bigcup_{k_n=1}^{p_n} \tilde{Z}_n^{k_n}$$
%
for the normalization of $X$, where $\tilde{Z}_j^{k_j}$ maps onto $Z_j$ under the normalization map $p: \tilde{X} \to X$. Choose points $u_i \in U_i$, $z_j \in Z_j$ and points $\tilde{u}_i \in \tilde{U}_i$, $\tilde{z}^{k_j}_j \in \tilde{Z}^{k_j}_j$ lying over $u_i$ and $z_j$. If $Z_j \subset \partial U_i$, then $\tilde{U}_i \cup \tilde{Z}_j^{k_j}$ is a smooth, irreducible $G$-chain. Choose fastening data $(\gamma_{i,j,k_j}, \ell_{i,j,k_j})$ for $(\tilde{U}_i,\tilde{Z}_j^{k_j})$ and write $G^s|_0(i,j,k_j), G^{\tame}_0(i,j,k_j)$, and $G^{\tame}_1(i,j,k_j)$ for the subgroups of $G$ defined in Subsection \ref{sec:univtame}. Recall, there is a diagram (of groups):
%
\begin{center}
\begin{tikzcd}
\stab_G(\ell_{i,j,k_j}(0)) & &  \stab_G(\ell_{i,j,k_j}(1)) \ar[d,twoheadrightarrow] \\
G^s|_0(i,j,k_j) \ar[u,hookrightarrow] \ar[r]& G_0^{\tame}(i,j,k_j) \ar[r,hookrightarrow] & G^{\tame}_1(i,j,k_j)
\end{tikzcd}
\end{center}
%
and hence a diagram (of abelian groups)
%
\begin{center}
\begin{tikzcd}
\Char\left(\stab_G(\ell_{i,j,k_j}(0))\right) \ar[d] & &  \Char\left(\stab_G(\ell_{i,j,k_j}(1))\right) \\
\Char\left(G^s|_0(i,j,k_j)\right) & \Char\left(G_0^{\tame}(i,j,k_j)\right)\ar[l] & \Char\left(G_1^{\tame}(i,j,k_j)\right) \ar[l] \ar[u,hookrightarrow]
\end{tikzcd}
\end{center}
%
where $\Char(H)$ denotes the character group of $H$. Although, in general $\ell_{i,j,k_j}(0) \neq \tilde{z}_j^{k_j}$ and $\ell_{i,j,k_j}(1) \neq \tilde{u}_i$, there are canonical isomorphisms (implemented by elements of $G$)

$$\Char\left(\stab_G(\ell_{i,j,k_j}(0))\right) \simeq \Char\left(\stab_G(\tilde{z}_j^{k_j})\right) \qquad \Char\left(\stab_G(\ell_{i,j,k_j}(1))\right) \simeq \Char\left(\stab_G(\tilde{u}_i)\right)$$

\noindent Thus, we obtain a diagram (with canonically defined maps):
%
\begin{center}
\begin{tikzcd}
 \Char\left(\stab_G(\tilde{z}_j^{k_j})\right) \ar[d] & &  \Char\left(\stab_G(\tilde{u}_i)\right) \\
\Char\left(G^s|_0(i,j,k_j)\right) & \Char\left(G_0^{\tame}\right)\ar[l] & \Char\left(G^1_{\tame}(i,j,k_j)\right) \ar[l] \ar[u,hookrightarrow]
\end{tikzcd}
\end{center}
%
Let 

$$\Psi_{i,j,k_j}: \Char\left(G^1_{\tame}(i,j,k_j)\right) \to \Char\left(G^s|_0(i,j,k_j)\right)$$

\noindent be the composition of the two horizontal maps in the diagram above. We call $\Psi_{i,j,k_j}$ the \emph{nearby cycles map} associated to the pair $(\tilde{u}_i, \tilde{z}_j^{k_j})$ to emphasize the analogy with Beilinson's constr. The maps $\Psi_{i,j,k_j}$, which are computable in examples (see, e.g. ??), encode the relationship between the restriction $\mathcal{L}|_{U_i}$ of a $G$-equivariant line bundle to an open $G$-orbit $U_i$ and its restriction $\mathcal{L}|_{Z_j}$ to a closed $G$-orbit $Z_j$ in its boundary. 

\begin{defn}
Define the category $\mathcal{D}(X)$ as follows. An object in $\mathcal{D}(X)$ is a tuple $(\rho_i,\lambda_j,\eta_{i,j,k_j})$ consisting of
\begin{itemize}
    \item a character
    %
    $$\rho_i \in \bigcap_{\tilde{Z}^{k_j}_j \subset \partial \tilde{U}_i} \Char\left(G^{\tame}_1(i,j,k_j)\right) \subseteq \Char\left(\stab_G(\tilde{u_i})\right)$$
    %
    for each open $G$-orbit $\tilde{U}_i$ on $\tilde{X}$,
    \item a character 
    %
    $$\lambda_j \in \Char(\left(\stab_G(z_j))\right)$$ 
    %
    for each closed $G$-orbit $Z_j$ on $X$, and
    \item an isomorphism (of characters)
    %
    $$\eta_{i,j,k_j}: \lambda_j|_{G^s|_0(i,j,k_j)} \simeq \Psi_{i,j,k_j}(\rho_i)$$
    %
    for each $\tilde{Z}^{k_j}_j \subseteq \partial \tilde{U}_i$.
\end{itemize}
%
A morphism $(\rho_i,\lambda_j,\eta_{i,j,k_j}) \to (\rho_i',\lambda_j',\eta_{i,j,k_j}')$ is a tuple $(f_i,g_j)$ consisting of

\begin{itemize}
    \item a homomorphism $f_i: \rho_i \to \rho_i'$ of characters of $\stab_G(\tilde{u}_i)$, and
    \item a homorphism $g_j : \lambda_j \to \lambda_j'$ of characters of $\stab_G(z_j)$ such that
    \item the following diagram commutes
    
    \begin{center}
    \begin{tikzcd}
    \lambda_j|_{G^s|_0(i,j,k_j)} \ar[d,"g_j"] \ar[r, "\eta_{i,j,k_j}"] & \Psi_{i,j,k_j}(\rho_i) \ar[d, "f_i"] \\
    \lambda_j'|_{G^s|_0(i,j,k_j)} \ar[r, "\eta'_{i,j,k_j}"] & \Psi_{i,j,k_j}(\rho'_i)
    \end{tikzcd}
    \end{center}
\end{itemize}
\end{defn}


\begin{prop}\label{prop:linebundles2}
There is a natural equivalence of categories
%
$$\Pic^G(X) \simeq \mathcal{D}(X)$$
\end{prop}


\begin{proof}
This is an easy consequence of Proposition \ref{prop:linebundles} combined with Proposition \ref{weak-prop-2}.
\end{proof}
\end{comment}
